Prompting Robot Teams with Natural Language

This paper presents a framework to prompt multi-robot teams with high-level tasks using natural language expressions. Our objective is to use the reasoning capabilities of language models in understanding and decomposing multi-robot collaboration and decision-making tasks, but in settings where such models cannot be called at deployment time. However, it is hard to specify the behavior of an individual robot from a team instruction, and have it continuously adapt to actions from other robots. This necessitates a framework with the representational capacity required by the logic and semantics of a task, and yet supports decentralized, real-time operation. We solve this dilemma by recognizing that a task can be represented as a deterministic finite automaton, and that recurrent neural networks (RNNs) can encode numerous automata. This allows us to distill the logic and sequential decompositions of sub-tasks obtained from a language model into an RNN, and align its internal states with the semantics of a given task. This leads to a tiny model that encapsulates the reasoning of the language model and can be implemented onboard. To interpret the internal state of the RNN for a decentralized execution, we train a graph neural network control policy conditioned on the hidden states of the RNN and the language embeddings. We present evaluations on simulated and real-world multi-robot tasks that require sequential and collaborative behavior by the team, demonstrating scalable, robust, real-time performance -- sites.google.com/view/prompting-teams.

==> rnn-task-model.tex <==
% \begin{figure}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tikzpicture}[
%   font=\rmfamily\footnotesize,
%   >=Latex,
%   node distance=4mm and 6mm,
%   every path/.style={line width=0.6pt},
%   io/.style={draw, rounded corners=2pt, minimum width=10mm, minimum height=6mm, align=center},
%   nn/.style={draw, ellipse, minimum width=18mm, minimum height=9mm, align=center},
%   loss/.style={draw, diamond, aspect=2, minimum width=10mm, align=center},
%   dbx/.style={dashed, very thick},
%   lab/.style={inner sep=1pt, font=\scriptsize}
% ]
% %\draw[help lines,step=2.5mm,gray!70] (0,-2) grid (10,2);

% % Nodes
% \node[io] (events) {Events};
% \node[nn, right=8mm of events, minimum width=12mm, inner sep=1pt] (rnn) {RNN $f_{\psi}$};

% \node[io, below=8mm of rnn] (taskemb) {High-level Task\\Embedding};

% \node[nn, right=11mm of rnn, minimum width=22mm] (stdec) {$d^{\text{class}}_{\phi}\left(x_{k}\right)$};
% \node[loss, right=6mm of stdec, , minimum width=16mm] (xce1) {$\mathcal{L}_{\text{class}}$};
% \node[io, above=6mm of xce1] (slab) {State label};

% \node[nn, dbx, below=7mm of stdec, minimum width=21mm] (ptdec) {$d^{\text{recon}}\left(x_{k}\right)$};
% \node[loss, right=6mm of ptdec, minimum width=16mm] (xce2) {$\mathcal{L}_{\text{recon}}$};
% \node[io, below=6mm of xce2] (alab) {$d^{\text{recon}}(e^l_{t,k})$};

% % Merge to final loss
% \coordinate (mA) at ($(xce1.east)+(3mm,0)$);
% \coordinate (mB) at ($(xce2.east)+(3mm,0)$);
% \coordinate (mC) at ($(mA)!0.5!(mB) + (12mm,0)$);
% \node[loss] (loss) at (mC) {Loss};

% % Connections
% \draw[->] (events) -- node[lab, above] {$e_t$} (rnn);

% % RNN self-loop
% \coordinate (rout) at ($(rnn.east)+(5mm,0)$);
% \coordinate (routu) at ($(rnn.north)+(0,3.5mm)$);
% \draw[->] (rnn.east) -- node[lab, below] {$h_t$} (rout);
% \draw (rout) |- (routu);
% \draw[->] (routu) -- (rnn.north);

% % To decoders
% \draw[->] (rout) -- (stdec.west);
% \draw[->] (stdec) -- (xce1);
% \draw[->] (slab) -- (xce1);

% % Optional branch
% \draw[->] (rout) |- (ptdec.west);
% \draw[->] (ptdec) -- (xce2);
% \draw[->] (alab) -- (xce2);

% % Merge losses
% \draw (xce1.east) -- (mA);
% \draw (xce2.east) -- (mB);
% \draw (mA) -- (mB);
% \draw[->] ($(mA)!0.5!(mB)$) -- (loss.west);

% % Task embedding into RNN
% \draw[->] (taskemb) -- node[lab, left] {$\mathcal{W}^l_{t}$} (rnn.south);

% \end{tikzpicture}%
% }
% \caption{Supervised training pipeline for the RNN task model.}
% \label{fig:rnn_training_pipeline}
% \end{figure}

% \begin{figure}[h]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tikzpicture}[
%   font=\rmfamily\footnotesize,
%   >=Latex,
%   node distance=4mm and 6mm,
%   every path/.style={line width=0.6pt},
%   io/.style={draw, rounded corners=2pt, minimum width=10mm, minimum height=6mm, align=center},
%   nn/.style={draw, ellipse, minimum width=18mm, minimum height=9mm, align=center},
%   loss/.style={draw, diamond, aspect=2, minimum width=10mm, align=center},
%   dbx/.style={dashed, very thick},
%   lab/.style={inner sep=1pt, font=\scriptsize}
% ]
% %\draw[help lines,step=2.5mm,gray!70] (0,-2) grid (10,2);

% % Nodes
% \node[io] (events) {Events};
% \node[nn, right=8mm of events, minimum width=12mm, inner sep=1pt] (rnn) {RNN $f_{\psi}$};

% \node[io, below=8mm of rnn] (taskemb) {High-level Task\\Embedding};

% \node[nn, right=11mm of rnn, minimum width=22mm] (stdec) {$d_{\phi}$};
% \node[loss, right=6mm of stdec, , minimum width=16mm] (xce1) {$\mathcal{L}$};
% \node[io, above=6mm of xce1] (slab) {State label};


% % Connections
% \draw[->] (events) -- node[lab, above] {$p^l_{i,k}$} (rnn);

% % RNN self-loop
% \coordinate (rout) at ($(rnn.east)+(5mm,0)$);
% \coordinate (routu) at ($(rnn.north)+(0,3.5mm)$);
% \draw[->] (rnn.east) -- node[lab, below] {$x_k$} (rout);
% \draw (rout) |- (routu);
% \draw[->] (routu) -- (rnn.north);

% % To decoders
% \draw[->] (rout) -- (stdec.west);
% \draw[->] (stdec) -- (xce1);
% \draw[->] (slab) -- (xce1);

% % Task embedding into RNN
% \draw[->] (taskemb) -- node[lab, left] {$\mathcal{E}^l_{i}$} (rnn.south);

% \end{tikzpicture}%
% }
% \caption{Supervised training pipeline for the RNN task model.}
% \label{fig:rnn_training_pipeline}
% \end{figure}

\begin{figure}[ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}[
  font=\rmfamily\footnotesize,
  >=Latex,
  node distance=4mm and 6mm,
  every path/.style={line width=0.6pt},
  io/.style={draw, rounded corners=2pt, minimum width=10mm, minimum height=3mm, align=center,font=\scriptsize},
  nn/.style={draw, ellipse, minimum width=18mm, minimum height=9mm, align=center},
  nn2/.style={draw, trapezium, trapezium angle=70, rotate=90, minimum width=12mm, minimum height=5mm, align=center},
  loss/.style={draw, diamond, aspect=2, minimum width=10mm, align=center},
  dbx/.style={dashed, very thick},
  lab/.style={inner sep=1pt, font=\scriptsize}
]
%\draw[help lines,step=2.5mm,gray!70] (0,-2) grid (10,2);

% Nodes
\node[io] (events) {Events};
\node[nn, right=8mm of events, minimum width=12mm, inner sep=1pt] (rnn) {RNN $f_{\psi}$};

\node[io, below=6mm of rnn] (taskemb) {High-level Task\\Embedding};

\node[nn2, right=11mm of rnn, minimum width=7mm,anchor=north] (stdec) {\rotatebox{-90}{$d_{\phi}$}};
\node[loss, right=24mm of rnn, minimum width=12mm,anchor=west] (xce1) {$\mathcal{L}$};
\node[io, above=6mm of xce1] (slab) {State label};


% Connections
\draw[->] (events) -- node[lab, above] {$p^l_{i,k}$} (rnn);

% RNN self-loop
\coordinate (rout) at ($(rnn.east)+(5mm,0)$);
\coordinate (routu) at ($(rnn.north)+(0,3.5mm)$);
\draw[->] (rnn.east) -- node[lab, below] {$x_k$} (rout);
\draw (rout) |- (routu);
\draw[->] (routu) -- (rnn.north);

% To decoders
\draw[->] (rout) -- (stdec.north);
\draw[->] (stdec) -- node[lab, above] {$\hat{h}^l_{i,k}$} (xce1.west); % Label added here
\draw[->] (slab) -- node[lab, left] {$h^l_{i,k}$} (xce1); % Label added here

% Task embedding into RNN
\draw[->] (taskemb) -- node[lab, left] {$\mathcal{E}^l_{i}$} (rnn.south);

\end{tikzpicture}%
}
\caption{Supervised training pipeline for the RNN task model.}
\label{fig:rnn_training_pipeline}
\end{figure}
